InsMapper: Exploring Inner-instance Information for Vectorized HD Mapping

Vectorized high-definition (HD) maps contain detailed information about surrounding road elements, which are crucial for various downstream tasks in modern autonomous vehicles, such as motion planning and vehicle control. Recent works attempt to directly detect the vectorized HD map as a point set prediction task, achieving notable detection performance improvements. However, these methods usually overlook and fail to analyze the important inner-instance correlations between predicted points, impeding further advancements. To address this issue, we investigate the utilization of inner-instance information for vectorized high-definition mapping through transformers, and propose a powerful system named $\textbf{InsMapper}$, which effectively harnesses inner-instance information with three exquisite designs, including hybrid query generation, inner-instance query fusion, and inner-instance feature aggregation. The first two modules can better initialize queries for line detection, while the last one refines predicted line instances. InsMapper is highly adaptable and can be seamlessly modified to align with the most recent HD map detection frameworks. Extensive experimental evaluations are conducted on the challenging NuScenes and Argoverse 2 datasets, where InsMapper surpasses the previous state-of-the-art method, demonstrating its effectiveness and generality. The project page for this work is available at https://tonyxuqaq.github.io/InsMapper/ .

==> figures/fig_anchor.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
  \centering
  \label{anchor}
  \begin{minipage}{\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/reference_baseline.png}
    \subcaption{No query fusion}
    \includegraphics[width=\linewidth]{imgs/reference_InsightMapper.png}
    \subcaption{With query fusion}
 \end{minipage}
  \caption{Predicted reference points for deformable DETR. Without query fusion, points within the same instance cannot see each other, thus they cannot generate complicated shapes, making all instances simple straight lines. With query fusion, the predicted reference points have a more similar distribution to the vector map elements, which enhances the final performance. }
  \label{reference}
\end{wrapfigure}

==> figures/fig_class_head.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/class_head.pdf}
  \caption{Class head designs. MapTR leverages the mean of points for aggregation (upper). While InsightMapper uses concatenation (lower). }
  \label{fig:class_head}
\end{wrapfigure}

==> figures/fig_inner_inter.tex <==
\begin{wrapfigure}{r}{0.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/inner_inter.pdf}
  \caption{Correlations between points. Inner-instance correlation (green lines) exists within the same instance, which benefits the detection performance. Inter-instance correlation (red lines) does not cast helpful constraints thus it should be blocked.}
  \label{inner-inter}
\end{wrapfigure}

==> figures/fig_ins_self_attn.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  % \vspace{-23pt}
  \includegraphics[width=\linewidth]{imgs/ins_self_attn.pdf}
  \caption{Decoder of InsMapper. An inner-instance multi-head self-attention module is incorporated into decoder layers. In this module, the attention between points belonging to different instances is blocked (grey grids). Only inner-instance attention is allowed (colored grids). Colored grids are randomly blocked with $\epsilon$ probability (set to grey) for robustness. The proposed module can further utilize inner-instance information and refine the predicted lines.}
  \label{ins_self_attn}
  \vspace{-20pt}
\end{wrapfigure}

==> figures/fig_inter_self_attn.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/inter_self_attn.pdf}
  \caption{Decoder of InsightMapper with inter-instance self-attention module. 
  In this module (the pink one), the attention between points of non-adjacent instances is blocked (grey grids). The attention is allowed for points of adjacent instances (pink grids), and diagonal grids (blue grids) to maintain the ego information of each point.}
  \label{fig:inter_self_attn}
  \vspace{-25pt}
\end{wrapfigure}

==> figures/fig_pos_ins_attn.tex <==
\begin{figure}[t]
  \centering
  \label{anchor}
  \begin{minipage}{0.21\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/1_v.pdf}
    \subcaption{Raw decoder}
    \end{minipage}
    \begin{minipage}{0.21\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/2_v.pdf}
    \subcaption{InsightMapper}
    \end{minipage}
    \begin{minipage}{0.21\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/3_v.pdf}
    \subcaption{Variant 1}
    \end{minipage}\\
    \begin{minipage}{0.21\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/4_v.pdf}
    \subcaption{Variant 2}
    \end{minipage}
  \begin{minipage}{0.21\linewidth}
  \centering
    \includegraphics[width=\linewidth]{imgs/5_v.pdf}
    \subcaption{Variant 3}
    \end{minipage}
     \begin{minipage}{0.21\linewidth}
    \includegraphics[width=\linewidth]{imgs/6_v.pdf}
    \subcaption{Variant 4}
    \end{minipage}
     \begin{minipage}{0.21\linewidth}
    \includegraphics[width=\linewidth]{imgs/7_v.pdf}
    \subcaption{Variant 5}
 \end{minipage}
  \caption{Different transformer decoder designs. (a) Raw decoder of the deformable DETR. (b) InsightMapper decoder. The proposed inner-instance self-attention module (blue) is incorporated. (c) Decoder variant 1. We replace the inner-instance self-attention module with a vanilla self-attention module. (d) Decoder variant 2. The self-attention module is removed from the InsightMapper decoder. (e) Decoder variant 3. Swap the inner-instance self-attention module with the cross-attention module of the variant 2. (f) Variant 4. Place the inner-instance self-attention module before the cross-attention module. (g) Variant 5. Place the inner-instance self-attention module before the self-attention module. InsightMapper decoder is the best design. Changing the structure of the proposed decoder will degrade the final performance.
}
  \label{fig:pos_ins_attn}
\end{figure}

==> figures/fig_vis_1.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{imgs/0.pdf}
%   \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
%   \label{fig:vis_1}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{imgs/0.pdf}
%   \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
%   \label{fig:vis_1}
% \end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/1.pdf}
  \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
  \label{fig:vis_2}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/2.pdf}
  \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
  \label{fig:vis_3}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/3.pdf}
  \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
  \label{fig:vis_4}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/4.pdf}
  \caption{Qualitative visualization. Left three columns are input 6 RGB camera images. For map columns, the first column presents MapTR's results, the second column features InsightMapper's outcomes, and the final column depicts the ground truth map. The predicted map contains four classes, i.e., road boundaries (green), lane splits (red), pedestrian crossing (blue), and lane centerlines (pink).}
  \label{fig:vis_5}
\end{figure}

==> tabs/tab_ablation_1.tex <==
\begin{table}[h]
  \caption{Quantitative results of comparison experiments on the NuScenes \textit{val} set. \textit{QF} represents the query fusion module; \textit{FA} means the maksed inner-instance self-attention module. For all metrics, a larger value indicates better performance.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{ablation_main}
  \centering
  \begin{tabular}{cccccccccc}
    \toprule
    \textit{QF} & \textit{FA} & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO & APLS  \\
    \midrule
    
     
    \checkmark &   & 43.28 & 47.27 & 50.77 & 40.47 & 45.45 &  &  \\
    
      
    & \checkmark& 41.95 & 51.69 & \textbf{53.52} & 40.55 & 46.93  &  &  \\

    \checkmark&\checkmark \textbf{44.36}& \textbf{53.36} & 52.77 & \textbf{42.35} & \textbf{48.31} &  &  \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_dn_detr.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies about denoising DETR. For all metrics, a larger value indicates better performance.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_dn_detr}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Method & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO  \\
    \midrule

     InsightMapper-Dn-DETR   &43.74&51.34&54.48&42.33&47.97{\color{myred}\tiny{($\downarrow$0.34)}}&50.37{\color{myred}\tiny{($\downarrow$1.21)}}  \\
     
      InsightMapper & 44.36& 53.36 & 52.77 & 42.35 & 48.31 & 51.58  \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_dynamic_query.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies about dynamic queries.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_dynamic_query}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Method & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO  \\
    \midrule

     InsightMapper with dynamic query & 43.14 & 48.86 &  52.17 & 38.65 & 45.71{\color{myred}\tiny{($\downarrow$2.60)}} & 43.83{\color{myred}\tiny{($\downarrow$7.75)}}  \\
      InsightMapper & 44.36& 53.36 & 52.77 & 42.35 & 48.31 &  51.58\\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_inter_instance.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies about inter-instance self-attention.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_inter_instance}
  \centering
  \begin{tabular}{llllllll}
    \toprule
    Inter-instance Self-attn & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO &  FPS    \\
    \midrule
    Yes &  42.40 & 53.21 & 54.03 & 43.03 & 48.17{\color{myred}\tiny{($\downarrow$0.14)}}  & 52.63{\color{mygreen}\tiny{($\uparrow$1.05)}} & 6.3 \\
     No (InsightMapper) & 44.36& 53.36 & 52.77 & 42.35 & 48.31 & 51.58 & 7.7 \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_mask.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies about the mask ratio.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_mask}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    $\epsilon$ & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO \\
    \midrule
    
     0 (No masked attn) & 42.48 & 50.66 & 53.22 & 41.54 & 46.98{\color{myred}\tiny{($\downarrow$1.33)}} & 51.49{\color{myred}\tiny{($\downarrow$0.09)}} \\
     
     25\% (InsightMapper) & 44.36& 53.36 & 52.77 & 42.35 & 48.31 &  51.58 \\
     
    50\% &  43.67&  52.57 &  53.98 & 42.95 & 48.17{\color{myred}\tiny{($\downarrow$0.14)}}  & 51.59{\color{mygreen}\tiny{($\uparrow$0.01)}} \\
    
      80\%  & 42.27 & 52.49 & 53.64 & 41.34 & 47.41{\color{myred}\tiny{($\downarrow$0.90)}} &  49.20{\color{myred}\tiny{($\downarrow$2.38)}} \\
      
    
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_modality.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies on multi-modality (camera and LiDAR).}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_modality}
  \centering
  \begin{tabular}{lcllllll}
    \toprule
    Method & Modality &$\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO \\
    \midrule
    
     MapTR  & C&  37.92 & 46.25 & 50.07 & 37.47 & 42.93 & 46.77 \\
     
     
     InsightMapper & C & {44.36} & {53.36} & {52.77} & {42.35} & {48.31} & {51.58}\\

     MapTR & C \& L &  49.47 & 58.98 & 66.72 & 44.89 & 55.01 & 56.77  \\


     InsightMapper & C \& L & 56.00 & 63.42 & 71.61 & 52.85 & 60.97{\color{mygreen}\tiny{($\uparrow$5.96)}} & 62.51{\color{mygreen}\tiny{($\uparrow$5.74)}}\\

    
     
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_pos_of_ins_attn.tex <==
\begin{table}[t]
  \caption{Quantitative results of ablation studies about transformer decoder architectures.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_pos_of_ins_attn}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Position & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO   \\
    \midrule
    Raw Decoder (No ins-self-attention) & 39.41 & 50.04 & 52.13 & 40.10 & 45.42{\color{myred}\tiny{($\downarrow$2.89)}} & 49.19{\color{myred}\tiny{($\downarrow$2.39)}} \\
    
 Variant 1 (Normal attention) & 40.50 & 50.78 & 52.17 & 41.46 & 46.23{\color{myred}\tiny{($\downarrow$2.08)}} & 49.51{\color{myred}\tiny{($\downarrow$1.41)}}  \\
    Variant 2 & 40.96 & 47.85 & 51.11 & 40.45 & 45.09{\color{myred}\tiny{($\downarrow$3.22)}} & 47.98{\color{myred}\tiny{($\downarrow$3.60)}} \\
   
     Variant 3 & 40.92 & 46.40 & 51.94 & 38.91 & 44.54{\color{myred}\tiny{($\downarrow$3.77)}} & 46.90{\color{myred}\tiny{($\downarrow$4.68)}} \\
     Variant 4 &  39.09 & 50.09 & 51.56 & 40.21 & 45.24{\color{myred}\tiny{($\downarrow$3.07)}}  & 48.16{\color{myred}\tiny{($\downarrow$3.42)}} \\
     
    Variant 5 & 44.04 &  49.59 & 52.18 & 41.78 & 46.90{\color{myred}\tiny{($\downarrow$1.41)}} & 49.52{\color{myred}\tiny{($\downarrow$2.06)}} \\
    InsightMapper & 44.36& 53.36 & 52.77 & 42.35 & 48.31 & 51.58 \\
      
    
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_post_processing.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies about post-processing threshold.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{ablation_pos_processing}
  \centering
  \begin{tabular}{ll}
    \toprule
    Threshold &  TOPO  \\
    \midrule
    
     None (No post-processing) &   \\

     0.05   & \\
     0.1 (InsightMapper)   & \\
     
    0.2 &   \\
    
      
      
    
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_ablation_query_generation.tex <==
\begin{table}[t]
  \caption{Quantitative results of ablation studies about query generation. For all metrics, a larger value indicates better performance.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{ablation_query_generation}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Query Generation Scheme & mAP & TOPO  \\
    \midrule
    
     MapTR  & 42.93{\color{myred}\tiny{($\downarrow$5.38)}} & 41.87{\color{myred}\tiny{($\downarrow$5.12)}}  \\
     InsightMapper-naive & 47.62{\color{myred}\tiny{($\downarrow$0.69)}}  & 46.33{\color{myred}\tiny{($\downarrow$0.76)}} \\
     InsightMapper-hierarchical &  46.93{\color{myred}\tiny{($\downarrow$1.38)}}  &  45.32{\color{myred}\tiny{($\downarrow$1.77)}} \\
     
    
    
      InsightMapper-hybrid &  \textbf{48.31} & \textbf{47.09}    \\
      
    
    \bottomrule
  \end{tabular}
\end{table} 

==> tabs/tab_class_head.tex <==
\begin{table}[h]
  \caption{Quantitative results of ablation studies on the class head design.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_class_head}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Aggregation Method & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO \\
    \midrule
    
     Mean & 42.31 & 53.22 & 53.70 & 43.16 & 48.10{\color{myred}\tiny{($\downarrow$0.21)}} & 51.19{\color{myred}\tiny{($\downarrow$0.39)}} \\
     
     Concatenation (InsightMapper) &   44.36& 53.36 & 52.77 & 42.35 & 48.31 & 51.58 \\
     
    
      
    
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_compare_maptr_v2_av2.tex <==
\begin{table}[!h]
  \caption{Quantitative results of comparison experiments on the Argoverse 2 \textit{validation} set. ``*" represents InsightMapper is enhanced by techniques leveraged in MapTR-V2. }
  \renewcommand\tabcolsep{2.5pt} 
  \small
  \label{tab:maptr_v2_av2}
  \centering
  \begin{tabular}{lccllllll}
    \toprule
    Methods & Epochs & Backbone & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO  \\
    \midrule
    
    % \midrule
    MapTR-V2  & 6 & R50 & 57.16 & 67.96 & 65.25 & 63.20 & 63.39 & 77.94\\
    % MapTR  & 110 & R18 &  \\
    InsightMapper* & 6 & R50 & \textbf{58.91}{\color{mygreen}\tiny{($\uparrow$1.75)}} & \textbf{71.35}{\color{mygreen}\tiny{($\uparrow$3.39)}} & \textbf{66.90}{\color{mygreen}\tiny{($\uparrow$1.65)}} & \textbf{64.70}{\color{mygreen}\tiny{($\uparrow$1.50)}} & \textbf{65.46}{\color{mygreen}\tiny{($\uparrow$2.07)}} & \textbf{79.26}{\color{mygreen}\tiny{($\uparrow$1.32)}}   \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_compare_maptrv2.tex <==
\begin{table}[t]
  \caption{Quantitative results of comparison experiments on the NuScenes \textit{validation} set. ``*" represents InsightMapper is enhanced by techniques leveraged in MapTR-V2. }
  \renewcommand\tabcolsep{2.4pt} 
  \small
  \label{tab:maptr_v2}
  \centering
  \begin{tabular}{lccllllll}
    \toprule
    Methods & Epochs & Backbone & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO  \\
    \midrule
    
    % \midrule
    MapTR-V2  & 24 & R50 & 48.20 & 54.75 & 56.66 & 45.86 & 51.37 & 51.15\\
    % MapTR  & 110 & R18 &  \\
    InsightMapper* & 24 & R50 & \textbf{49.07}{\color{mygreen}\tiny{($\uparrow$0.87)}} & \textbf{57.98}{\color{mygreen}\tiny{($\uparrow$3.23)}} & \textbf{59.84}{\color{mygreen}\tiny{($\uparrow$3.18)}} & \textbf{47.99}{\color{mygreen}\tiny{($\uparrow$2.13)}} & \textbf{53.72}{\color{mygreen}\tiny{($\uparrow$2.35)}} & \textbf{53.00}{\color{mygreen}\tiny{($\uparrow$1.85)}}   \\
    \midrule
    MapTR-V2  & 110 & R50 & 58.68 & 65.72 & 67.12 & 56.16 & 61.92 & 63.26\\
    
    % InsightMapper & 24 & R18 & \\
    
    InsightMapper* & 110 & R50 & \textbf{62.09}{\color{mygreen}\tiny{($\uparrow$3.41)}} & \textbf{67.60}{\color{mygreen}\tiny{($\uparrow$1.88)}} & \textbf{68.15}{\color{mygreen}\tiny{($\uparrow$1.03)}} & \textbf{58.41}{\color{mygreen}\tiny{($\uparrow$2.25)}} & \textbf{64.06}{\color{mygreen}\tiny{($\uparrow$2.14)}} & \textbf{64.72}{\color{mygreen}\tiny{($\uparrow$1.46)}}\\
    % InsightMapper & 24 & R101 &  &  &  &  &  &  &\\
    % InsightMapper & 110 & R101 &  &  &  &  &  &  &  \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_directed_graph.tex <==
\begin{table}[h]
  \caption{Quantitative results of different data representations (centerlines are directed graph).}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{tab:ablation_directed}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Method & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO  \\
    \midrule
    
     
    MapTR  & 37.39 & 46.61 & 50.69 & 37.22 & 42.98 & 46.98  \\
    
      
    InsightMapper & 43.24 & 53.77 & 53.89 & 43.22 & 48.53{\color{mygreen}\tiny{($\uparrow$5.55)}}  & 52.09{\color{mygreen}\tiny{($\uparrow$5.11)}}  \\

    \bottomrule
  \end{tabular}
\end{table}

==> tabs/tab_efficiency.tex <==
\begin{wraptable}{r}{0.45\textwidth}
  \caption{Efficiency of experiments on the NuScences \textit{val} set. Train represents training time per epoch (hour); test shows inference speed (FPS); size means the model weight size.}
  \renewcommand\tabcolsep{3pt} 
  \small
  \label{efficiency}
  \centering
  \begin{tabular}{lllll}
    \toprule
    Methods & Backbone & Train & Test &  Size  \\
    \midrule
    % HDMapNet & Effi-B0\\
    % STSU & R50\\
    % VectorMapNet & R50\\
    % MapTR & R18 &  & \\
    MapTR & R50 & 0.52h & 9.1 & 453M\\
    % InsightMapper & R18 & & \\
    InsightMapper & R50 & 0.53h & 9.1 & 580M \\
    \bottomrule
  \end{tabular}
\end{wraptable}

==> tabs/tab_num_decoder_layers.tex <==
\begin{table}[h]
  \caption{Quantitative results of comparison experiments on the NuScenes \textit{val} set. For all metrics, a larger value indicates better performance.}
  \small
   \renewcommand\tabcolsep{7pt} 
  \label{ablation_decoder_layer_num}
  \centering
  \begin{tabular}{cccccccccc}
    \toprule
    Number of decoder layers & $\text{AP}_{\text{\textit{ped}}}$ & $\text{AP}_{\text{\textit{div}}}$ & $\text{AP}_{\text{\textit{bound}}}$ & $\text{AP}_{\text{\textit{center}}}$ & mAP & TOPO & APLS  \\
    \midrule
    
     
     
     1 &    & \\
     3 &    & \\
     6 & \textbf{44.30} & \textbf{52.51} & 53.00 & \textbf{62.61} & \textbf{47.94} \\
    8 &    \\
    
      
    
    \bottomrule
  \end{tabular}
\end{table}
